Probing gravity with the DES-CMASS sample and BOSS spectroscopy

The DES-CMASS sample (DMASS) is designed to optimally combine the weak lensing measurements from the Dark Energy Survey (DES) and redshift-space distortions (RSD) probed by the CMASS galaxy sample from the Baryonic Oscillation Spectroscopic Survey (BOSS). In this paper, we demonstrate the feasibility of adopting DMASS as the equivalent of BOSS CMASS for a joint analysis of DES and BOSS in the framework of modified gravity. We utilize the angular clustering of the DMASS galaxies, cosmic shear of the DES METACALIBRATION sources, and cross-correlation of the two as data vectors. By jointly fitting the combination of the data with the RSD measurements from the BOSS CMASS sample and Planck data, we obtain the constraints on modified gravity parameters $\mu_0 = -0.37^{+0.47}_{-0.45}$ and $\Sigma_0 = 0.078^{+0.078}_{-0.082}$. We do not detect any significant deviation from General Relativity. Our constraints of modified gravity measured with DMASS are tighter than those with the DES Year 1 redMaGiC galaxy sample with the same external data sets by $29\%$ for $\mu_0$ and $21\%$ for $\Sigma_0$, and comparable to the published results of the DES Year 1 modified gravity analysis despite this work using fewer external data sets. This improvement is mainly because the galaxy bias parameter is shared and more tightly constrained by both CMASS and DMASS, effectively breaking the degeneracy between the galaxy bias and other cosmological parameters. Such an approach to optimally combine photometric and spectroscopic surveys using a photometric sample equivalent to a spectroscopic sample can be applied to combining future surveys having a limited overlap such as DESI and LSST.

==> Makefile <==
texfile := main
outputpdf := Lee_et_al_Producing_a_BOSS-CMASS_sample_with_DES_imaging.pdf

all:
	pdflatex ${texfile}
	bibtex ${texfile}
	bibtex ${texfile}
	pdflatex ${texfile}
	pdflatex ${texfile}
	pdflatex ${texfile}
	cp ${texfile}.pdf ${outputpdf}

bib: 
	bibtex ${texfile}
	bibtex ${texfile}

pdf: 
	pdflatex ${texfile}
	pdflatex ${texfile}

clean:
	rm -f \
	${texfile}.dvi \
	${texfile}.pdf \
	${texfile}.aux \
	${texfile}.bbl \
	${texfile}.blg \
	${texfile}.toc \
	${texfile}.log


==> authorlist_mnras.tex <==
% Author list file generated with: mkauthlist 1.2.3+16.gfd56256 
% mkauthlist -f -j mnras --sort-builder DES-2020-0532_author_list_sorted.csv authorlist_mnras.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
S.~Lee,$^{1}$\thanks{E-mail: sujeong.lee717@duke.edu}
E.~M.~Huff,$^{2}$
A.~Choi,$^{3}$
J.~Elvin-Poole,$^{3,4}$
C.~ Hirata,$^{3,4}$
K.~Honscheid,$^{3,4}$
N.~MacCrann,$^{5}$
A.~J.~Ross,$^{3}$
M.~A.~Troxel,$^{1}$
T.~F.~Eifler,$^{6,2}$
H.~ Kong,$^{3,4}$
J.~Blazek,$^{3,7}$
A.~Fert\'e,$^{2}$
D.~Huterer,$^{8}$
A.~Campos,$^{9}$
A.~Chen,$^{8}$
S.~Dodelson,$^{9}$
P.~Lemos,$^{10,11}$
C.~D.~Leonard,$^{12}$
V.~Miranda,$^{6}$
J.~Muir,$^{13}$
M.~Raveri,$^{14}$
L.~F.~Secco,$^{15}$
N.~Weaverdyck,$^{8}$
J.~Zuntz,$^{16}$
S.~L.~Bridle,$^{17}$
C.~Davis,$^{13}$
J.~DeRose,$^{18,19}$
M.~Gatti,$^{15}$
J.~Prat,$^{20}$
M.~M.~Rau,$^{9}$
S.~Samuroff,$^{9}$
C.~S{\'a}nchez,$^{15}$
P.~Vielzeuf,$^{21}$
M.~Aguena,$^{22,23}$
S.~Allam,$^{24}$
A.~Amon,$^{13}$
F.~Andrade-Oliveira,$^{25,23}$
G.~M.~Bernstein,$^{15}$
E.~Bertin,$^{26,27}$
D.~Brooks,$^{10}$
D.~L.~Burke,$^{13,28}$
A.~Carnero~Rosell,$^{29,23,30}$
M.~Carrasco~Kind,$^{31,32}$
J.~Carretero,$^{21}$
F.~J.~Castander,$^{33,34}$
R.~Cawthon,$^{35}$
C.~Conselice,$^{17,36}$
M.~Costanzi,$^{37,38,39}$
L.~N.~da Costa,$^{23,40}$
M.~E.~S.~Pereira,$^{8}$
J.~De~Vicente,$^{41}$
S.~Desai,$^{42}$
H.~T.~Diehl,$^{24}$
J.~P.~Dietrich,$^{43}$
P.~Doel,$^{10}$
S.~Everett,$^{19}$
A.~E.~Evrard,$^{44,8}$
I.~Ferrero,$^{45}$
P.~Fosalba,$^{33,34}$
J.~Frieman,$^{24,14}$
J.~Garc\'ia-Bellido,$^{46}$
E.~Gaztanaga,$^{33,34}$
D.~W.~Gerdes,$^{44,8}$
T.~Giannantonio,$^{47,48}$
D.~Gruen,$^{49,13,28}$
R.~A.~Gruendl,$^{31,32}$
J.~Gschwend,$^{23,40}$
G.~Gutierrez,$^{24}$
W.~G.~Hartley,$^{50}$
S.~R.~Hinton,$^{51}$
D.~L.~Hollowood,$^{19}$
B.~Hoyle,$^{43,52}$
D.~J.~James,$^{53}$
K.~Kuehn,$^{54,55}$
N.~Kuropatkin,$^{24}$
O.~Lahav,$^{10}$
M.~Lima,$^{22,23}$
M.~A.~G.~Maia,$^{23,40}$
M.~March,$^{15}$
J.~L.~Marshall,$^{56}$
F.~Menanteau,$^{31,32}$
R.~Miquel,$^{57,21}$
J.~J.~Mohr,$^{43,52}$
R.~Morgan,$^{35}$
A.~Palmese,$^{24,14}$
F.~Paz-Chinch\'{o}n,$^{31,47}$
A.~Pieres,$^{23,40}$
A.~A.~Plazas~Malag\'on,$^{58}$
A.~Roodman,$^{13,28}$
E.~Sanchez,$^{41}$
V.~Scarpine,$^{24}$
M.~Schubnell,$^{8}$
S.~Serrano,$^{33,34}$
I.~Sevilla-Noarbe,$^{41}$
E.~Sheldon,$^{59}$
M.~Smith,$^{60}$
E.~Suchyta,$^{61}$
M.~E.~C.~Swanson,$^{31}$
G.~Tarle,$^{8}$
D.~Thomas,$^{62}$
C.~To,$^{49,13,28}$
T.~N.~Varga,$^{52,63}$
and J.~Weller$^{52,63}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{2}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{3}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{4}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{5}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{6}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{7}$ Institute of Physics, Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland\\
$^{8}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{9}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{10}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{11}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{12}$ School of Mathematics, Statistics and Physics, Newcastle University, Newcastle upon Tyne, NE1 7RU, UK \\
$^{13}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{14}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{15}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{16}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{17}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{18}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{19}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{20}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{21}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{22}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{23}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{24}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{25}$ Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil\\
$^{26}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{27}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{28}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{29}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{30}$ Universidad de La Laguna, Dpto. Astrofisica, E-38206 La Laguna, Tenerife, Spain\\
$^{31}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{32}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{33}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{34}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{35}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{36}$ University of Nottingham, School of Physics and Astronomy, Nottingham NG7 2RD, UK\\
$^{37}$ Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy\\
$^{38}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{39}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{40}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{41}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{42}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{43}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{44}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{45}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{46}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{47}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{48}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{49}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{50}$ Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland\\
$^{51}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{52}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{53}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{54}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{55}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{56}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{57}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{58}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{59}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{60}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{61}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{62}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{63}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}

